Statistical mechanical theory of liquid water

Water is an unusual liquid. Its thermophysical properties are non-monotonic with temperature T and pressure p. It's not been known how water's behaviors are encoded in its molecules. We give a statistical physics model, Cage Water, which assumes three bonding states: van der Waals, pairwise hydrogen bonding, and multi-body cooperative caging hydrogen bonds. The model is analytical, so very fast to compute, yet it gives excellent agreement with extensive pT experiments. Through readily interpretable substates, Cage Water explains water's liquid anomalies -- including its controversial liquid-liquid supercooling transition -- as simple switchovers among the three bonding types.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
